Anomaly Detection through Transfer Learning in Agriculture and Manufacturing IoT Systems

IoT systems have been facing increasingly sophisticated technical problems due to the growing complexity of these systems and their fast deployment practices. Consequently, IoT managers have to judiciously detect failures (anomalies) in order to reduce their cyber risk and operational cost. While there is a rich literature on anomaly detection in many IoT-based systems, there is no existing work that documents the use of ML models for anomaly detection in digital agriculture and in smart manufacturing systems. These two application domains pose certain salient technical challenges. In agriculture the data is often sparse, due to the vast areas of farms and the requirement to keep the cost of monitoring low. Second, in both domains, there are multiple types of sensors with varying capabilities and costs. The sensor data characteristics change with the operating point of the environment or machines, such as, the RPM of the motor. The inferencing and the anomaly detection processes therefore have to be calibrated for the operating point. In this paper, we analyze data from sensors deployed in an agricultural farm with data from seven different kinds of sensors, and from an advanced manufacturing testbed with vibration sensors. We evaluate the performance of ARIMA and LSTM models for predicting the time series of sensor data. Then, considering the sparse data from one kind of sensor, we perform transfer learning from a high data rate sensor. We then perform anomaly detection using the predicted sensor data. Taken together, we show how in these two application domains, predictive failure classification can be achieved, thus paving the way for predictive maintenance.

==> Discussion.tex <==
\section{Discussion} \label{sec:Discussion}
% \name studies the effects of human behavioral decision making, represented by non-linear perceptions of probabilities, on the security of interdependent CPS. Addressing the impact of such effects would be an interesting question for further research in the security community. One possible solution is to guide security decision makers to invest in the critical edges (or min-cut edges) in their attack graph model of the CPS system. Also, encouraging cooperative defense and reducing selfish decisions would be another mitigation.

In this paper, we have studied the impacts of human behavioral decision making
%, represented by non-linear weighting of actual probabilities of attacks to determine human-perceived probabilities. We have seen through the various system configurations that different levels of loss may arise from behavioral decision making, 
to the security of the system overall and to individual stakeholders. We believe this opens up a new dimension of {\em intervention} in securing interdependent systems. How does one guide security decision makers to the appropriate levels of behavioral weighting (such as, the optimal value of $\alpha$ for a given protected system)? How does one incentivize multiple stakeholders to cooperate to achieve greater system-level security? What is the role of a centralized regulatory agency in incentivizing the security-beneficial investments by individual stakeholders? The last point has to be cognizant of different proprietary and regulatory pressures, which will limit knowledge sharing or ability to invest in another stakeholder's assets. Some recent work has explored how game theory can be used to analyze such situations, using the principle of hyper-games~\cite{gutierrez2018hypergame}. Further, another dominant factor of behavioral decision making is the loss aversion principle---a dollar lost is more painful than a dollar gained is pleasurable \cite{kahneman1991anomalies,thaler1997effect}. How does this play into securing interdependent systems? In our current formulation, since the defender tries to minimize her cost, there is no room for gain and therefore the loss aversion does not affect our model or insights. However, in other formulations, it may be needed. Finally, although we use the Prelec weighting function in our formulation, other probability weighting functions with similar properties e.g., Tversky-Kahneman (discussed in Appendix \ref{app: another_prob_model}) or the class discussed in \cite[Section II]{7544460}, can be used in our framework. %Finally, an alternative to the assumption of independent attack success across edges is to consider conditional probabilities of success throughout the path; this is a  challenging direction of future work. 
% SB (11/1/18): Chopped for space. We have already put a forward pointer to Tversky-Kahneman function in evaluation. 
% Mus(11/1/18): If reviewer doesn't read the appendix, he may raise the question that our formulation is only with 
%Prelec.

% Another point is although, we use Prelec weighting function in our formulation, other probability weighting functions with the same properties (e.g., Tversky-Kahneman (discussed in Appendix \ref{app: another_prob_model}) or the class discussed in (\cite{7544460}, Section II)) works also for our formulation. %Moreover, there are some classes of attack graphs where the suboptimal decision making may not happen (e.g. graphs with symmetric parallel sub-paths).  

%\saurabh{I reworded it above and please check if you agree.}
% \issa{I think it would be more appropriate to use the word "study" rather than "address". I do not know if you have addressed that behavior impact on security, which leads me to the question of how can the security community benefit from this study? or how can they use the insights and findings of this study to enhance the security posture of relevant systems.} 
% %For example, if we set the initial link probabilities into the inverse weighing function of the original initial probabilities, does this solve the problem all-in-all, as this maps the original problem with behavior defenders into a problem with non-behavioral defenders.}.
% \mustafa{
% I changed it to studies. One idea is to guide security analyst via a visualization tool that extracts min-cut edges from attack graph of the model and tell him to only invest in these edges.}
% However, probability weighting is not the only part in the prospect theory. For example, prospect theory showed that human weighs losses more than gains (i.e., human are sad for losses much than being happy for equivalent gains).  but that may not be the only possible realistic scenario.

% \section{Discussion} \label{sec:discussion}
% In some scenarios, the defenders are domain experts which may arise the question of being rational all the way. According to prospect theory, even if the defender is a domain expert, behavioral decision making show that the defender under risk would waste amount of money on non-critical edges. For example, in the DER.1 scenario, the defender would waste amount of her security budget into attack steps which are not critical. In this example, the critical attack step that need to be well mitigated is authentication and ensuring that the passwords are changed. However, according to classical model (i.e., rational defender), the player would go and spend all money on authentication. This shows that in some scenarios, the classical model may be more realistic. 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

